Diversified Ensembling: An Experiment in Crowdsourced Machine Learning

Crowdsourced machine learning on competition platforms such as Kaggle is a popular and often effective method for generating accurate models. Typically, teams vie for the most accurate model, as measured by overall error on a holdout set, and it is common towards the end of such competitions for teams at the top of the leaderboard to ensemble or average their models outside the platform mechanism to get the final, best global model. In arXiv:2201.10408, the authors developed an alternative crowdsourcing framework in the context of fair machine learning, in order to integrate community feedback into models when subgroup unfairness is present and identifiable. There, unlike in classical crowdsourced ML, participants deliberately specialize their efforts by working on subproblems, such as demographic subgroups in the service of fairness. Here, we take a broader perspective on this work: we note that within this framework, participants may both specialize in the service of fairness and simply to cater to their particular expertise (e.g., focusing on identifying bird species in an image classification task). Unlike traditional crowdsourcing, this allows for the diversification of participants' efforts and may provide a participation mechanism to a larger range of individuals (e.g. a machine learning novice who has insight into a specific fairness concern). We present the first medium-scale experimental evaluation of this framework, with 46 participating teams attempting to generate models to predict income from American Community Survey data. We provide an empirical analysis of teams' approaches, and discuss the novel system architecture we developed. From here, we give concrete guidance for how best to deploy such a framework.

==> bias-bounties-description.tex <==
For the purposes of our empirical study, we consider a competition for a regression problem. Formally, we consider the task of prediction over a distribution of labelled examples $\Z = \X \times \Y$, where $\X$ are features and $\Y \in \mathbb{R}$ are real-valued labels that will be predicted by a model $f$. Let $\D \in \Delta Z$ be the joint distribution over features and labels, and let $D \sim \D^n$ denote a finite set of $n$ labeled samples drawn i.i.d.\ from the distribution $\D$. We measure performance of the model $f$ by its mean squared error over the distribution, where the error for a single prediction $f(x)$ is defined as $\ell: \X \times Y \rightarrow \mathbb{R}; \ \ell(f(x), y)) = (f(x) - y)^2$, and average loss is denoted $\Loss(\D, f) = \mean_{(x,y) \sim \D} [\ell(f(x), y)]$. 

In \cite{globus2022algorithmic}, the authors propose an algorithmic framework termed a ``bias bounty" for iteratively patching a predictor $f$ when regions with provably suboptimal performance are identified by auditors. Formally, auditors are tasked with constructing $(g,h)$-pairs of functions: a \textit{group} indicator function $g : \mathcal{X} \to \{0,1\}$ and a \textit{hypothesis} predictor $h : \mathcal{X} \to \mathcal{Y}$. We define the group loss of a predictor $f$ on $g$ as $\Loss(\D, f, g) = \mean_{(x,y) \sim D}[(f(x)-y)^2 \vert g(x)=1]$. If a competitor is able to construct a $(g,h)$-pair such that $\Loss(\D, f,  g) > \Loss(\D, h, g)$, then the pair is \textit{accepted} and the model $f$ is \textit{updated}. 

The data structure for updating the model $f$ is a form of decision list with base node $f$: when a $(g,h)$ pair is accepted, a new decision node is prepended to the structure with group inclusion as the test on the prepended node. Then, the updated model $f'$ will predict $h(x)$ for all instances such that $g(x) = 1$, and $f(x)$ otherwise. We can iterate this process, allowing bounty hunters to search for new $(g,h)$-pairs to reduce performance error on $f'$. For notations sake, let $f_{0}$ denote the initial model before any updates have been made, let ($g_{i}, h_{i}$) denote the $i^{th}$ accepted pair to the model, and let $f_{i}$ denote the model after accepting $(g_{i}, h_{i})$. 

Since the proposed groups may not be disjoint, it is possible than an update $(g_{k}, h_{k})$ may improve performance on group $g_{k}$ while decreasing performance on an earlier group $g_{i}$ due to group intersections. In order to avoid this, the model is iteratively patched after updates: for each $g_{i}$ $i \leq j < k$, the model $f_{j}$ which performs best on $g_{i}$ tracked. After each update, if the model's error on any previously identified group has gotten worse, then the model is \textit{repaired} by prepending a node with test for group inclusion of $g_{i}$ which ``points" to $f_{j}$ if $g_{i} = 1$ and to $f_{k}$ otherwise. .\footnote{This is a slight deviation from the text of the MonotoneFalsifyAndUpdate procedure described in \cite{globus2022algorithmic}, but is morally equivalent and substantially faster.} This implies that once a $(g,h)$ pair is accepted into the overall model, the error rate on $g$ is non-increasing. We denote this as the ``repair" procedure. 

In practice, we cannot verify improvements or track the group losses necessary for repairs over distributional loss. Instead, a sample of validation data, not accessible by bounty hunters, is used to calculate all losses. Additionally, rather than unilateraly accepting any update that improves in error, the acceptance/repair criteria must require a decrease in overall error by some $\alpha > 0$. This is necessary in order to guarantee eventual convergence of the algorithm to the optimal model, and is necessary for the generalization guarantees of \cite{globus2022algorithmic}; see for example Theorems 12 and 14 in \cite{globus2022algorithmic}. \igh{Michael, Aaron, are you ok with just citing the theorems? Restating will require a lot of additional notation we haven't bothered w here.}

